GFDM Transceiver using Precoded Data and Low-complexity Multiplication in Time Domain

Future wireless communication systems are demanding a more flexible physical layer. GFDM is a block filtered multicarrier modulation scheme proposed to add multiple degrees of freedom and cover other waveforms in a single framework. In this paper, GFDM modulation and demodulation will be presented as a frequency-domain circular convolution, allowing for a reduction of the implementation complexity when MF, ZF and MMSE filters are employed in the inner and outer receiver operation. Also, precoding is introduced to further increase GFDM flexibility, addressing a wider set of applications.

==> 6.tex <==
\section{Conclusions}\label{sec:5}

\LLM{This paper introduces a GFDM modulator and demodulator based on a low-complexity multiplication in the time-domain. The new matrix model allows to consider the coefficients transmitted by the subcarriers as the precoding of the data symbols. This approach broadens the GFDM flexibility, allowing to use different transforms to achieve different goals. The computational complexity of the new scheme has been compared with the solution proposed in \cite{Gaspar2013}, showing that the modem solution proposed in this paper can reduce the number of complex valued multiplications, even when sparse filters in the frequency-domain are employed.}

